Advancing Dynamic Fault Tree Analysis

This paper presents a new state space generation approach for dynamic fault trees (DFTs) together with a technique to synthesise failures rates in DFTs. Our state space generation technique aggressively exploits the DFT structure --- detecting symmetries, spurious non-determinism, and don't cares. Benchmarks show a gain of more than two orders of magnitude in terms of state space generation and analysis time. Our approach supports DFTs with symbolic failure rates and is complemented by parameter synthesis. This enables determining the maximal tolerable failure rate of a system component while ensuring that the mean time of failure stays below a threshold.

==> dft-tikz.tex <==

\makeatletter

\pgfdeclareshape{spare}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{P}{ % primary anchor
    \pgf@process{\northeast}%
    \pgf@x=-.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SD}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{BOX}{ % spare box anchor
    \pgf@process{\northeast}%
    \pgf@x=\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@spare@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % Box for spare parts
    \pgf@anchor@spare@BOX
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.\pgf@y
    \advance\pgf@yb by -.8\pgf@y
    \advance\pgf@xb by -1\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{spare/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@spare@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}

    \pgf@anchor@spare@P 
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SD
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{spare/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every spare node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,fill=white!100!black,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\pgfdeclareshape{spareM}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{P}{ % primary anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SD}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=-.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{SE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{BOX}{ % spare box anchor
    \pgf@process{\northwest}%
    \pgf@x=\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@spare@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % Box for spare parts
    \pgf@anchor@spare@BOX
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.\pgf@y
    \advance\pgf@xa by -1\pgf@x
    \advance\pgf@yb by -.8\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{spareM/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@spare@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}

    \pgf@anchor@spare@P 
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SD
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@spare@SE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{spareM/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every spareM node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\pgfdeclareshape{fdep}{
  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]

  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  % Define anchors for signal ports
  \anchor{O}{ % output anchor
    \pgf@process{\northeast}%
    \pgf@x=0pt%
  }
  \anchor{EA}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.1\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EB}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.3\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EC}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{ED}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.7\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{EE}{ % spare anchor
    \pgf@process{\northeast}%
    \pgf@x=.9\pgf@x%
    \pgf@y=-\pgf@y%
  }
  \anchor{T}{ % trigger anchor
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{LINE}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.\pgf@y%
  }
  % Draw the rectangle box and the port labels
  \backgroundpath{
    % Rectangle box
    \pgfpathrectanglecorners{\southwest}{\northeast}
    % Line in the middle
    \pgf@anchor@fdep@LINE
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \advance\pgf@xb by -2\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    % trinagle input
    \pgf@anchor@fdep@T
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \advance\pgf@ya by -.3333\pgf@x
    \advance\pgf@xb by -.5\pgf@x
    \advance\pgf@yb by .\pgf@x
    \advance\pgf@yc by .3333\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    \pgfclosepath

    % Draw port labels
    \begingroup
    \tikzset{fdep/port labels} % Use font from this style
    \tikz@textfont

    \pgf@anchor@fdep@O
    \pgftext[top,at={\pgfpoint{\pgf@x}{\pgf@y}},y=-\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EA
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EB
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EC
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@ED
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    
    \pgf@anchor@fdep@EE
    \pgftext[bottom,at={\pgfpoint{\pgf@x}{\pgf@y}},y=\pgfshapeinnerysep]{}
    \endgroup
  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{fdep/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every fdep node/.style={draw,minimum height=1cm,minimum 
width=1.5cm,inner sep=1mm,outer sep=0pt,cap=round,add 
font=\sffamily}}

\newif\ifpgfshapebaselesstrianglehasinline
\newif\ifpgfshapebaselesstriangleclose
\pgfkeys{/pgf/.cd,
  baseless triangle apex angle/.style={/pgf/isosceles triangle apex angle=#1},
  baseless triangle inline/.is if=pgfshapebaselesstrianglehasinline,
  baseless triangle has base/.is if=pgfshapebaselesstriangleclose
}

\pgfdeclareshape{baseless triangle}{
  % Copy some stuff from the isosecles triangle
  \inheritsavedanchors[from={isosceles triangle}]
  \inheritanchor[from={isosceles triangle}]{center}
  \inheritanchor[from={isosceles triangle}]{north}
  \inheritanchor[from={isosceles triangle}]{south}
  \inheritanchor[from={isosceles triangle}]{east}
  \inheritanchor[from={isosceles triangle}]{west}
  \inheritanchorborder[from={isosceles triangle}]
  \backgroundpath{%
    % The isoceles triangle defines lots of parameters
    % in the \trianglepoints macro.
        \trianglepoints%
        {%
            \pgftransformshift{\centerpoint}%
            \pgftransformrotate{\rotate}%
            % This bit is a bit of a kludge to ensure the inline
            % is at the top of the figure.
            \pgftransformyscale{cos(\rotate)}%
            \pgfpathmoveto{\lowerleft}%
            \pgfpathlineto{\apex}%
            \pgfpathlineto{\lowerleft\pgf@y=-\pgf@y}%
            % Close the base?
            \ifpgfshapebaselesstriangleclose%
              \pgfpathclose%
            \fi%
            % Draw the inline?
            \ifpgfshapebaselesstrianglehasinline
              \pgfpointdiff{\lowerleft}%
                 {\pgfpointlineattime{0.125}{\lowerleft}{\lowerleft\pgf@y=-\pgf@y}}%
                \pgfgetlastxy{\x}{\y}%
                \pgfmathveclen{\x}{\y}%
                \let\inlineshift=\pgfmathresult%
            % Calculate where the inline hits the sloped line of the triangle.
            \pgfmathparse{\inlineshift/2/sin(\pgfkeysvalueof{/pgf/isosceles triangle apex angle}/2)}%
            \let\inlineendshift=\pgfmathresult
            \pgfpathmoveto{\pgfpointadd{\pgfpoint{0pt}{-\inlineshift}}{\lowerleft}}%
            \pgfpathlineto{\pgfpointlineatdistance{\inlineendshift}{\apex}{\lowerleft}\pgf@y=-\pgf@y}%
        \fi%
    }
    }
}





\makeatother

\tikzstyle{every picture}=[>=stealth]
\tikzstyle{fdarrow}=[>=triangle 60,double,double equal sign distance,-implies,dashed]
\tikzstyle{and1}=[and gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=n,minimum width=1cm]
\tikzstyle{and2}=[and gate US,draw,  shape border rotate=90, rotate=90,logic gate inputs=nn,minimum width=1cm]
\tikzstyle{and3}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{and}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{and4}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnn,minimum width=1cm, scale=0.9]
\tikzstyle{and5}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{and6}=[and gate US,draw, shape border rotate=90, rotate=90,logic gate inputs=nnnnnn,minimum width=1cm, scale=0.7]
\tikzstyle{or1}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=n,minimum width=1cm]
\tikzstyle{or2}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nn,minimum width=1cm]
\tikzstyle{or3}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{or}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnn,minimum width=1cm]
\tikzstyle{or4}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnn,minimum width=1cm, scale=0.9]
\tikzstyle{or5}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{or6}=[or gate US,draw,shape border rotate=90, rotate=90,logic gate inputs=nnnnnn,minimum width=1cm, scale=0.8]
\tikzstyle{be}=[circle,draw,fill=white!100,anchor=north, inner sep=5pt, minimum width=0.7cm]
\tikzstyle{cnst}=[diamond,draw,fill=white!100,anchor=north, minimum width=0.5cm,font=\scriptsize, scale=0.8]
\tikzstyle{seq}=[rectangle,draw,fill=white!100, minimum width=0.7cm,font=\LARGE, inner sep=3pt]
\tikzstyle{labelbox} = [rectangle, draw, inner sep=2pt, anchor=south, minimum width=0.6cm, minimum height=0.4cm, scale=0.8]
\tikzstyle{transfer} = [isosceles triangle, draw, shape border rotate=90, inner sep=2pt, minimum width=0.9cm, minimum height=0.7cm, isosceles triangle stretches=true]

\tikzstyle{triangle}=[isosceles triangle,draw,shape border rotate=90,isosceles triangle stretches=true, minimum height=0.6cm,minimum width=0.6cm]
\tikzstyle{btriangle}=[baseless triangle,draw,rotate=90, minimum height=0.6cm]
